Learning to Evaluate the Artness of AI-generated Images

Assessing the artness of AI-generated images continues to be a challenge within the realm of image generation. Most existing metrics cannot be used to perform instance-level and reference-free artness evaluation. This paper presents ArtScore, a metric designed to evaluate the degree to which an image resembles authentic artworks by artists (or conversely photographs), thereby offering a novel approach to artness assessment. We first blend pre-trained models for photo and artwork generation, resulting in a series of mixed models. Subsequently, we utilize these mixed models to generate images exhibiting varying degrees of artness with pseudo-annotations. Each photorealistic image has a corresponding artistic counterpart and a series of interpolated images that range from realistic to artistic. This dataset is then employed to train a neural network that learns to estimate quantized artness levels of arbitrary images. Extensive experiments reveal that the artness levels predicted by ArtScore align more closely with human artistic evaluation than existing evaluation metrics, such as Gram loss and ArtFID.

==> tables/quantitative.tex <==
\begin{table*}[t]
\scriptsize
\centering
\caption{The correlation between the ranking induced by the user study conducted in~\cite{wright2022artfid} and the ranking induced by ArtScore and other metrics based on three aggregation methods, as given by Eq.~\ref{equ:rank}, Eq.~\ref{equ:add}, and Eq.~\ref{equ:mul}. For the ArtFID metric, we report the result in~\cite{wright2022artfid}(paper), and the re-implemented result using the stylized images generated in our experiments (rep). The highest correlation is highlighted in bold, and the second highest is underlined.}
\label{table:correlation result}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|lc|lc|lc}
\hline
\multirow{2}{*}{\textbf{Aspects}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Metrics}}} & \multicolumn{2}{c|}{\textbf{Rank}} & \multicolumn{2}{c|}{\textbf{Add}} & \multicolumn{2}{c}{\textbf{Multiply}} \\\cline{3-8}
 & \multicolumn{1}{c|}{} & \textbf{Spearman’s \bm{$\rho$} ↑} & \textbf{\textit{p}-value ↓} & \textbf{Spearman’s \bm{$\rho$} ↑} & \textbf{\textit{p}-value ↓} &  \textbf{Spearman’s \bm{$\rho$} ↑} & \textbf{\textit{p}-value ↓} \\\hline
Artness & ArtScore & 0.6364 & 0.0261 & 0.6364 & 0.0261 & 0.6364 & 0.0261 \\\hline
\multirow{3}{*}{Style} & Gram Loss & -0.3286 & 0.2969 & -0.3286 & 0.2969 & -0.3286 & 0.2969 \\\cline{2-8}
 & ArtFID\_Style & 0.6504 & 0.0220 & 0.6504 & 0.0220 & 0.6504 & 0.0220 \\
 & \hspace{3mm}+ArtScore & 0.7549 (\textcolor{red}{+0.1045}) & 0.0045 & 0.7483 (\textcolor{red}{+0.0979}) & 0.0051 & \underline{0.7972} (\textcolor{red}{+0.1468}) & \underline{0.0019} \\\hline
\multirow{8}{*}{Content} & LPIPS & 0.4126 & 0.1826 & 0.4126 & 0.1826 & 0.4126 & 0.1826 \\
 & \hspace{3mm}+ArtScore & 0.7138 (\textcolor{red}{+0.3012}) & 0.0091 & 0.5385 (\textcolor{red}{+0.1259}) & 0.0709 & 0.5175 (\textcolor{red}{+0.1049}) & 0.0849 \\\cline{2-8}
 & Content Loss & 0.4755 & 0.1182 & 0.4755 & 0.1182 & 0.4755 & 0.1182 \\
 & \hspace{3mm}+ArtScore & 0.5835 (\textcolor{red}{+0.1080}) & 0.0464 & 0.6084 (\textcolor{red}{+0.1329}) & 0.0358 & 0.6084 (\textcolor{red}{+0.1329}) & 0.0358 \\\cline{2-8}
 & SSIM & 0.5315 & 0.0754 & 0.5315 & 0.0754 & 0.5315 & 0.0754 \\
 & \hspace{3mm}+ArtScore & 0.5965 (\textcolor{red}{+0.0650}) & 0.0406 & 0.5594 (\textcolor{red}{+0.0269}) & 0.0586 & 0.5594 (\textcolor{red}{+0.0279}) & 0.0586 \\\cline{2-8}
 & L2 & 0.2837 & 0.3715 & 0.2837 & 0.3715 & 0.2837 & 0.3715 \\
 & \hspace{3mm}+ArtScore & 0.5298 (\textcolor{red}{+0.2461}) & 0.0764 & 0.5874 (\textcolor{red}{+0.3037}) & 0.0446 & 0.5874 (\textcolor{red}{+0.3037}) & 0.0446 \\\hhline{========}
\multirow{11}{*}{Style+Content} & ArtFID$\infty$ (paper) & 0.9301* & 0.0000* & 0.9301* & 0.0000* & 0.9301* & 0.0000* \\\cline{2-8}
 & ArtFID$\infty$ (rep) & 0.7063 & 0.0102 & 0.7063 & 0.0102 & 0.7063 & 0.0102 \\
 & \hspace{3mm}+ArtScore & 0.7790 (\textcolor{red}{+0.0727}) & 0.0028 & \underline{0.7552} (\textcolor{red}{+0.0489}) & \underline{0.0045} & \textbf{0.8182} (\textcolor{red}{+0.1045}) & \textbf{0.1119} \\\cline{2-8}
 & ArtFID\_Style+LPIPS & 0.6714 & 0.0168 & 0.6550 & 0.0208 & 0.7063 & 0.0102 \\
 & \hspace{3mm}+ArtScore & 0.7552 (\textcolor{red}{+0.0838}) & 0.0045 & \textbf{0.7902} (\textcolor{red}{+0.1352}) & \textbf{0.0022} & \textbf{0.8182} (\textcolor{red}{+0.1119}) & \textbf{0.0011} \\\cline{2-8}
 & ArtFID\_Style+Content Loss & 0.7874 & 0.0024 & 0.6504 & 0.0220 & 0.7483 & 0.0051 \\
 & \hspace{3mm}+ArtScore & \textbf{0.8196} (\textcolor{red}{+0.0322}) & \textbf{0.0011} & \textbf{0.7902} (\textcolor{red}{+0.1398}) & \textbf{0.0022} & \underline{0.7972} (\textcolor{red}{+0.0489}) & \underline{0.0019} \\\cline{2-8}
 & ArtFID\_Style+SSIM & \underline{0.8120} & \underline{0.0013} & 0.6573 & 0.0202 & \underline{0.7972} & \underline{0.0019} \\
 & \hspace{3mm}+ArtScore & 0.7719 (\textcolor{black}{-0.0401}) & 0.0033 & \textbf{0.7902} (\textcolor{red}{+0.1329}) & \textbf{0.0022} & \textbf{0.8182} (\textcolor{red}{+0.0210}) & \textbf{0.0011} \\\cline{2-8}
 & ArtFID\_Style+L2 & 0.6843 & 0.0141 & 0.6573 & 0.0202 & 0.7483 & 0.0051 \\
 & \hspace{3mm}+ArtScore & 0.7356 (\textcolor{red}{+0.0513}) & 0.0064 & 0.7483 (\textcolor{red}{+0.0910}) & 0.0051 & 0.7692 (\textcolor{red}{+0.0209}) & 0.0034 \\\hline
\end{tabular}
}
  \vspace{-0.2in}
\end{table*}
